Differentiable-by-design Nonlinear Optimization for Model Predictive Control

Nonlinear optimization-based control policies, such as those arising in nonlinear Model Predictive Control, have seen remarkable success in recent years. These policies require solving computationally demanding nonlinear optimization programs online at each time-step. The resulting solution map, viewed as a function of the measured state of the system and design parameters, may not be differentiable, which poses significant challenges if the control policy is embedded in a gradient-based policy optimization scheme. We propose a principled way to regularize the nonlinear optimization problem around the nominal solution, obtaining a surrogate derivative even if the solution map of the original problem is not differentiable. The surrogate problem is differentiable by design and its solution coincides with the solution of the unregularized problem. We demonstrate the effectiveness of our approach in a free-final-time optimal control problem and a receding-horizon nonlinear MPC example.

==> Figures/Data/a.tex <==
t v
0.0000000000e+00 -9.9999999999e-01
1.6765524759e-02 -9.9999999999e-01
3.3531049519e-02 -9.9999999999e-01
5.0296574278e-02 -9.9999999999e-01
6.7062099037e-02 -9.9999999999e-01
8.3827623796e-02 -9.9999999999e-01
1.0059314856e-01 -9.9999999999e-01
1.1735867331e-01 -9.9999999999e-01
1.3412419807e-01 -9.9999999999e-01
1.5088972283e-01 -9.9999999999e-01
1.6765524759e-01 -9.9999999999e-01
1.8442077235e-01 -9.9999999999e-01
2.0118629711e-01 -9.9999999999e-01
2.1795182187e-01 -9.9999999999e-01
2.3471734663e-01 -9.9999999999e-01
2.5148287139e-01 -9.9999999999e-01
2.6824839615e-01 -9.9999999998e-01
2.8501392091e-01 -9.9999999998e-01
3.0177944567e-01 -9.9999999998e-01
3.1854497043e-01 -9.9999999998e-01
3.3531049519e-01 -9.9999999997e-01
3.5207601994e-01 -9.9999999996e-01
3.6884154470e-01 -9.9999999994e-01
3.8560706946e-01 -9.9999999988e-01
4.0237259422e-01 -5.0352476701e-01
4.1913811898e-01 9.9999999988e-01
4.3590364374e-01 9.9999999994e-01
4.5266916850e-01 9.9999999996e-01
4.6943469326e-01 9.9999999997e-01
4.8620021802e-01 9.9999999998e-01
5.0296574278e-01 9.9999999998e-01
5.1973126754e-01 9.9999999998e-01
5.3649679230e-01 9.9999999998e-01
5.5326231706e-01 9.9999999999e-01
5.7002784182e-01 9.9999999999e-01
5.8679336657e-01 9.9999999999e-01
6.0355889133e-01 9.9999999999e-01
6.2032441609e-01 9.9999999999e-01
6.3708994085e-01 9.9999999999e-01
6.5385546561e-01 9.9999999999e-01
6.7062099037e-01 9.9999999999e-01
6.8738651513e-01 9.9999999999e-01
7.0415203989e-01 9.9999999999e-01
7.2091756465e-01 9.9999999999e-01
7.3768308941e-01 9.9999999999e-01
7.5444861417e-01 9.9999999999e-01
7.7121413893e-01 9.9999999999e-01
7.8797966369e-01 9.9999999999e-01
8.0474518844e-01 9.9999999999e-01
8.2151071320e-01 9.9999999999e-01
8.3827623796e-01 9.9999999999e-01
8.5504176272e-01 9.9999999999e-01
8.7180728748e-01 9.9999999999e-01
8.8857281224e-01 9.9999999999e-01
9.0533833700e-01 9.9999999999e-01
9.2210386176e-01 9.9999999999e-01
9.3886938652e-01 9.9999999999e-01
9.5563491128e-01 9.9999999999e-01
9.7240043604e-01 9.9999999999e-01
9.8916596080e-01 9.9999999999e-01
1.0059314856e+00 9.9999999999e-01
1.0226970103e+00 9.9999999999e-01
1.0394625351e+00 9.9999999999e-01
1.0562280598e+00 9.9999999999e-01
1.0729935846e+00 9.9999999999e-01
1.0897591094e+00 9.9999999999e-01
1.1065246341e+00 9.9999999999e-01
1.1232901589e+00 9.9999999999e-01
1.1400556836e+00 9.9999999998e-01
1.1568212084e+00 9.9999999998e-01
1.1735867331e+00 9.9999999998e-01
1.1903522579e+00 9.9999999998e-01
1.2071177827e+00 9.9999999998e-01
1.2238833074e+00 9.9999999998e-01
1.2406488322e+00 9.9999999998e-01
1.2574143569e+00 9.9999999998e-01
1.2741798817e+00 9.9999999998e-01
1.2909454065e+00 9.9999999998e-01
1.3077109312e+00 9.9999999998e-01
1.3244764560e+00 9.9999999998e-01
1.3412419807e+00 9.9999999998e-01
1.3580075055e+00 9.9999999998e-01
1.3747730303e+00 9.9999999998e-01
1.3915385550e+00 9.9999999998e-01
1.4083040798e+00 9.9999999998e-01
1.4250696045e+00 9.9999999998e-01
1.4418351293e+00 9.9999999998e-01
1.4586006541e+00 9.9999999998e-01
1.4753661788e+00 9.9999999998e-01
1.4921317036e+00 9.9999999997e-01
1.5088972283e+00 9.9999999997e-01
1.5256627531e+00 9.9999999997e-01
1.5424282779e+00 9.9999999997e-01
1.5591938026e+00 9.9999999997e-01
1.5759593274e+00 9.9999999996e-01
1.5927248521e+00 9.9999999995e-01
1.6094903769e+00 9.9999999993e-01
1.6262559016e+00 9.9999999989e-01
1.6430214264e+00 9.9999999978e-01
1.6597869512e+00 -8.2335169857e-02
1.6765524759e+00 -9.9999999977e-01
1.6933180007e+00 -9.9999999989e-01
1.7100835254e+00 -9.9999999992e-01
1.7268490502e+00 -9.9999999994e-01
1.7436145750e+00 -9.9999999995e-01
1.7603800997e+00 -9.9999999996e-01
1.7771456245e+00 -9.9999999996e-01
1.7939111492e+00 -9.9999999997e-01
1.8106766740e+00 -9.9999999997e-01
1.8274421988e+00 -9.9999999997e-01
1.8442077235e+00 -9.9999999997e-01
1.8609732483e+00 -9.9999999997e-01
1.8777387730e+00 -9.9999999998e-01
1.8945042978e+00 -9.9999999998e-01
1.9112698226e+00 -9.9999999998e-01
1.9280353473e+00 -9.9999999998e-01
1.9448008721e+00 -9.9999999998e-01
1.9615663968e+00 -9.9999999998e-01
1.9783319216e+00 -9.9999999998e-01
1.9950974464e+00 -9.9999999998e-01
2.0118629711e+00 -9.9999999998e-01
2.0286284959e+00 -9.9999999998e-01
2.0453940206e+00 -9.9999999998e-01
2.0621595454e+00 -9.9999999998e-01
2.0789250701e+00 -9.9999999998e-01
2.0956905949e+00 -9.9999999999e-01
2.1124561197e+00 -9.9999999999e-01
2.1292216444e+00 -9.9999999999e-01
2.1459871692e+00 -9.9999999999e-01
2.1627526939e+00 -9.9999999999e-01
2.1795182187e+00 -9.9999999999e-01
2.1962837435e+00 -9.9999999999e-01
2.2130492682e+00 -9.9999999999e-01
2.2298147930e+00 -9.9999999999e-01
2.2465803177e+00 -9.9999999999e-01
2.2633458425e+00 -9.9999999999e-01
2.2801113673e+00 -9.9999999999e-01
2.2968768920e+00 -9.9999999999e-01
2.3136424168e+00 -9.9999999999e-01
2.3304079415e+00 -9.9999999999e-01
2.3471734663e+00 -9.9999999999e-01
2.3639389911e+00 -9.9999999999e-01
2.3807045158e+00 -9.9999999999e-01
2.3974700406e+00 -9.9999999999e-01
2.4142355653e+00 -9.9999999999e-01
2.4310010901e+00 -9.9999999999e-01
2.4477666149e+00 -9.9999999999e-01
2.4645321396e+00 -9.9999999999e-01
2.4812976644e+00 -9.9999999999e-01
2.4980631891e+00 -9.9999999999e-01
2.5148287139e+00 -9.9999999999e-01


==> Figures/Data/a_m2.tex <==
t v
0.0000000000e+00 -9.9999999999e-01
1.6437986647e-02 -9.9999999999e-01
3.2875973294e-02 -9.9999999999e-01
4.9313959940e-02 -9.9999999999e-01
6.5751946587e-02 -9.9999999999e-01
8.2189933234e-02 -9.9999999999e-01
9.8627919881e-02 -9.9999999999e-01
1.1506590653e-01 -9.9999999999e-01
1.3150389317e-01 -9.9999999999e-01
1.4794187982e-01 -9.9999999999e-01
1.6437986647e-01 -9.9999999999e-01
1.8081785312e-01 -9.9999999999e-01
1.9725583976e-01 -9.9999999999e-01
2.1369382641e-01 -9.9999999999e-01
2.3013181306e-01 -9.9999999999e-01
2.4656979970e-01 -9.9999999999e-01
2.6300778635e-01 -9.9999999998e-01
2.7944577300e-01 -9.9999999998e-01
2.9588375964e-01 -9.9999999998e-01
3.1232174629e-01 -9.9999999998e-01
3.2875973294e-01 -9.9999999997e-01
3.4519771958e-01 -9.9999999996e-01
3.6163570623e-01 -9.9999999994e-01
3.7807369288e-01 -9.9999999988e-01
3.9451167952e-01 5.8520779094e-01
4.1094966617e-01 9.9999999988e-01
4.2738765282e-01 9.9999999994e-01
4.4382563946e-01 9.9999999996e-01
4.6026362611e-01 9.9999999997e-01
4.7670161276e-01 9.9999999997e-01
4.9313959940e-01 9.9999999998e-01
5.0957758605e-01 9.9999999998e-01
5.2601557270e-01 9.9999999998e-01
5.4245355935e-01 9.9999999999e-01
5.5889154599e-01 9.9999999999e-01
5.7532953264e-01 9.9999999999e-01
5.9176751929e-01 9.9999999999e-01
6.0820550593e-01 9.9999999999e-01
6.2464349258e-01 9.9999999999e-01
6.4108147923e-01 9.9999999999e-01
6.5751946587e-01 9.9999999999e-01
6.7395745252e-01 9.9999999999e-01
6.9039543917e-01 9.9999999999e-01
7.0683342581e-01 9.9999999999e-01
7.2327141246e-01 9.9999999999e-01
7.3970939911e-01 9.9999999999e-01
7.5614738575e-01 9.9999999999e-01
7.7258537240e-01 9.9999999999e-01
7.8902335905e-01 9.9999999999e-01
8.0546134569e-01 9.9999999999e-01
8.2189933234e-01 9.9999999999e-01
8.3833731899e-01 9.9999999999e-01
8.5477530564e-01 9.9999999999e-01
8.7121329228e-01 9.9999999999e-01
8.8765127893e-01 9.9999999999e-01
9.0408926558e-01 9.9999999999e-01
9.2052725222e-01 9.9999999999e-01
9.3696523887e-01 9.9999999999e-01
9.5340322552e-01 9.9999999999e-01
9.6984121216e-01 9.9999999999e-01
9.8627919881e-01 9.9999999999e-01
1.0027171855e+00 9.9999999999e-01
1.0191551721e+00 9.9999999999e-01
1.0355931588e+00 9.9999999999e-01
1.0520311454e+00 9.9999999998e-01
1.0684691320e+00 9.9999999998e-01
1.0849071187e+00 9.9999999998e-01
1.1013451053e+00 9.9999999998e-01
1.1177830920e+00 9.9999999998e-01
1.1342210786e+00 9.9999999998e-01
1.1506590653e+00 9.9999999998e-01
1.1670970519e+00 9.9999999998e-01
1.1835350386e+00 9.9999999998e-01
1.1999730252e+00 9.9999999998e-01
1.2164110119e+00 9.9999999998e-01
1.2328489985e+00 9.9999999998e-01
1.2492869852e+00 9.9999999998e-01
1.2657249718e+00 9.9999999998e-01
1.2821629585e+00 9.9999999998e-01
1.2986009451e+00 9.9999999998e-01
1.3150389317e+00 9.9999999998e-01
1.3314769184e+00 9.9999999998e-01
1.3479149050e+00 9.9999999998e-01
1.3643528917e+00 9.9999999998e-01
1.3807908783e+00 9.9999999997e-01
1.3972288650e+00 9.9999999997e-01
1.4136668516e+00 9.9999999997e-01
1.4301048383e+00 9.9999999997e-01
1.4465428249e+00 9.9999999997e-01
1.4629808116e+00 9.9999999997e-01
1.4794187982e+00 9.9999999997e-01
1.4958567849e+00 9.9999999997e-01
1.5122947715e+00 9.9999999997e-01
1.5287327582e+00 9.9999999996e-01
1.5451707448e+00 9.9999999995e-01
1.5616087314e+00 9.9999999993e-01
1.5780467181e+00 9.9999999989e-01
1.5944847047e+00 9.9999999979e-01
1.6109226914e+00 8.3066111093e-01
1.6273606780e+00 -9.9999999978e-01
1.6437986647e+00 -9.9999999989e-01
1.6602366513e+00 -9.9999999992e-01
1.6766746380e+00 -9.9999999994e-01
1.6931126246e+00 -9.9999999995e-01
1.7095506113e+00 -9.9999999996e-01
1.7259885979e+00 -9.9999999997e-01
1.7424265846e+00 -9.9999999997e-01
1.7588645712e+00 -9.9999999997e-01
1.7753025579e+00 -9.9999999997e-01
1.7917405445e+00 -9.9999999998e-01
1.8081785312e+00 -9.9999999998e-01
1.8246165178e+00 -9.9999999998e-01
1.8410545044e+00 -9.9999999998e-01
1.8574924911e+00 -9.9999999998e-01
1.8739304777e+00 -9.9999999998e-01
1.8903684644e+00 -9.9999999998e-01
1.9068064510e+00 -9.9999999998e-01
1.9232444377e+00 -9.9999999998e-01
1.9396824243e+00 -9.9999999998e-01
1.9561204110e+00 -9.9999999998e-01
1.9725583976e+00 -9.9999999998e-01
1.9889963843e+00 -9.9999999998e-01
2.0054343709e+00 -9.9999999998e-01
2.0218723576e+00 -9.9999999998e-01
2.0383103442e+00 -9.9999999999e-01
2.0547483309e+00 -9.9999999999e-01
2.0711863175e+00 -9.9999999999e-01
2.0876243041e+00 -9.9999999999e-01
2.1040622908e+00 -9.9999999999e-01
2.1205002774e+00 -9.9999999999e-01
2.1369382641e+00 -9.9999999999e-01
2.1533762507e+00 -9.9999999999e-01
2.1698142374e+00 -9.9999999999e-01
2.1862522240e+00 -9.9999999999e-01
2.2026902107e+00 -9.9999999999e-01
2.2191281973e+00 -9.9999999999e-01
2.2355661840e+00 -9.9999999999e-01
2.2520041706e+00 -9.9999999999e-01
2.2684421573e+00 -9.9999999999e-01
2.2848801439e+00 -9.9999999999e-01
2.3013181306e+00 -9.9999999999e-01
2.3177561172e+00 -9.9999999999e-01
2.3341941038e+00 -9.9999999999e-01
2.3506320905e+00 -9.9999999999e-01
2.3670700771e+00 -9.9999999999e-01
2.3835080638e+00 -9.9999999999e-01
2.3999460504e+00 -9.9999999999e-01
2.4163840371e+00 -9.9999999999e-01
2.4328220237e+00 -9.9999999999e-01
2.4492600104e+00 -9.9999999999e-01
2.4656979970e+00 -9.9999999999e-01


==> Figures/Data/a_m2_approx.tex <==
t v
0.0000000000e+00 -9.9999999999e-01
1.6420657654e-02 -9.9999999999e-01
3.2841315307e-02 -9.9999999999e-01
4.9261972961e-02 -9.9999999999e-01
6.5682630615e-02 -9.9999999999e-01
8.2103288268e-02 -9.9999999999e-01
9.8523945922e-02 -9.9999999999e-01
1.1494460358e-01 -9.9999999999e-01
1.3136526123e-01 -9.9999999999e-01
1.4778591888e-01 -9.9999999999e-01
1.6420657654e-01 -9.9999999999e-01
1.8062723419e-01 -9.9999999999e-01
1.9704789184e-01 -9.9999999999e-01
2.1346854950e-01 -9.9999999999e-01
2.2988920715e-01 -9.9999999999e-01
2.4630986480e-01 -9.9999999999e-01
2.6273052246e-01 -9.9999999998e-01
2.7915118011e-01 -9.9999999998e-01
2.9557183777e-01 -9.9999999998e-01
3.1199249542e-01 -9.9999999998e-01
3.2841315307e-01 -9.9999999997e-01
3.4483381073e-01 -9.9999999996e-01
3.6125446838e-01 -9.9999999994e-01
3.7767512603e-01 -9.9999999988e-01
3.9409578369e-01 6.0558028975e-01
4.1051644134e-01 9.9999999988e-01
4.2693709899e-01 9.9999999994e-01
4.4335775665e-01 9.9999999996e-01
4.5977841430e-01 9.9999999997e-01
4.7619907196e-01 9.9999999998e-01
4.9261972961e-01 9.9999999998e-01
5.0904038726e-01 9.9999999998e-01
5.2546104492e-01 9.9999999998e-01
5.4188170257e-01 9.9999999999e-01
5.5830236022e-01 9.9999999999e-01
5.7472301788e-01 9.9999999999e-01
5.9114367553e-01 9.9999999999e-01
6.0756433318e-01 9.9999999999e-01
6.2398499084e-01 9.9999999999e-01
6.4040564849e-01 9.9999999999e-01
6.5682630615e-01 9.9999999999e-01
6.7324696380e-01 9.9999999999e-01
6.8966762145e-01 9.9999999999e-01
7.0608827911e-01 9.9999999999e-01
7.2250893676e-01 9.9999999999e-01
7.3892959441e-01 9.9999999999e-01
7.5535025207e-01 9.9999999999e-01
7.7177090972e-01 9.9999999999e-01
7.8819156737e-01 9.9999999999e-01
8.0461222503e-01 9.9999999999e-01
8.2103288268e-01 9.9999999999e-01
8.3745354034e-01 9.9999999999e-01
8.5387419799e-01 9.9999999999e-01
8.7029485564e-01 9.9999999999e-01
8.8671551330e-01 9.9999999999e-01
9.0313617095e-01 9.9999999999e-01
9.1955682860e-01 9.9999999999e-01
9.3597748626e-01 9.9999999999e-01
9.5239814391e-01 9.9999999999e-01
9.6881880156e-01 9.9999999999e-01
9.8523945922e-01 9.9999999999e-01
1.0016601169e+00 9.9999999999e-01
1.0180807745e+00 9.9999999999e-01
1.0345014322e+00 9.9999999999e-01
1.0509220898e+00 9.9999999999e-01
1.0673427475e+00 9.9999999999e-01
1.0837634051e+00 9.9999999999e-01
1.1001840628e+00 9.9999999999e-01
1.1166047204e+00 9.9999999998e-01
1.1330253781e+00 9.9999999998e-01
1.1494460358e+00 9.9999999998e-01
1.1658666934e+00 9.9999999998e-01
1.1822873511e+00 9.9999999998e-01
1.1987080087e+00 9.9999999998e-01
1.2151286664e+00 9.9999999998e-01
1.2315493240e+00 9.9999999998e-01
1.2479699817e+00 9.9999999998e-01
1.2643906393e+00 9.9999999998e-01
1.2808112970e+00 9.9999999998e-01
1.2972319546e+00 9.9999999998e-01
1.3136526123e+00 9.9999999998e-01
1.3300732699e+00 9.9999999998e-01
1.3464939276e+00 9.9999999998e-01
1.3629145853e+00 9.9999999998e-01
1.3793352429e+00 9.9999999998e-01
1.3957559006e+00 9.9999999998e-01
1.4121765582e+00 9.9999999998e-01
1.4285972159e+00 9.9999999998e-01
1.4450178735e+00 9.9999999998e-01
1.4614385312e+00 9.9999999997e-01
1.4778591888e+00 9.9999999997e-01
1.4942798465e+00 9.9999999997e-01
1.5107005041e+00 9.9999999997e-01
1.5271211618e+00 9.9999999997e-01
1.5435418194e+00 9.9999999996e-01
1.5599624771e+00 9.9999999995e-01
1.5763831347e+00 9.9999999993e-01
1.5928037924e+00 9.9999999989e-01
1.6092244501e+00 9.9999999978e-01
1.6256451077e+00 -1.1972920311e+00
1.6420657654e+00 -9.9999999977e-01
1.6584864230e+00 -9.9999999989e-01
1.6749070807e+00 -9.9999999992e-01
1.6913277383e+00 -9.9999999994e-01
1.7077483960e+00 -9.9999999995e-01
1.7241690536e+00 -9.9999999996e-01
1.7405897113e+00 -9.9999999996e-01
1.7570103689e+00 -9.9999999997e-01
1.7734310266e+00 -9.9999999997e-01
1.7898516842e+00 -9.9999999997e-01
1.8062723419e+00 -9.9999999997e-01
1.8226929996e+00 -9.9999999997e-01
1.8391136572e+00 -9.9999999998e-01
1.8555343149e+00 -9.9999999998e-01
1.8719549725e+00 -9.9999999998e-01
1.8883756302e+00 -9.9999999998e-01
1.9047962878e+00 -9.9999999998e-01
1.9212169455e+00 -9.9999999998e-01
1.9376376031e+00 -9.9999999998e-01
1.9540582608e+00 -9.9999999998e-01
1.9704789184e+00 -9.9999999998e-01
1.9868995761e+00 -9.9999999998e-01
2.0033202337e+00 -9.9999999998e-01
2.0197408914e+00 -9.9999999998e-01
2.0361615491e+00 -9.9999999998e-01
2.0525822067e+00 -9.9999999999e-01
2.0690028644e+00 -9.9999999999e-01
2.0854235220e+00 -9.9999999999e-01
2.1018441797e+00 -9.9999999999e-01
2.1182648373e+00 -9.9999999999e-01
2.1346854950e+00 -9.9999999999e-01
2.1511061526e+00 -9.9999999999e-01
2.1675268103e+00 -9.9999999999e-01
2.1839474679e+00 -9.9999999999e-01
2.2003681256e+00 -9.9999999999e-01
2.2167887832e+00 -9.9999999999e-01
2.2332094409e+00 -9.9999999999e-01
2.2496300985e+00 -9.9999999999e-01
2.2660507562e+00 -9.9999999999e-01
2.2824714139e+00 -9.9999999999e-01
2.2988920715e+00 -9.9999999999e-01
2.3153127292e+00 -9.9999999999e-01
2.3317333868e+00 -9.9999999999e-01
2.3481540445e+00 -9.9999999999e-01
2.3645747021e+00 -9.9999999999e-01
2.3809953598e+00 -9.9999999999e-01
2.3974160174e+00 -9.9999999999e-01
2.4138366751e+00 -9.9999999999e-01
2.4302573327e+00 -9.9999999999e-01
2.4466779904e+00 -9.9999999999e-01
2.4630986480e+00 -9.9999999999e-01


==> Figures/Data/position_params.tex <==
\def\dubinsTf{2.514829}%


==> Figures/Data/s.tex <==
t v
0.0000000000e+00 -3.2382636614e-02
1.6765524759e-02 -9.9999999963e-01
3.3531049519e-02 -9.9999999983e-01
5.0296574278e-02 -9.9999999989e-01
6.7062099037e-02 -9.9999999992e-01
8.3827623796e-02 -9.9999999994e-01
1.0059314856e-01 -9.9999999995e-01
1.1735867331e-01 -9.9999999996e-01
1.3412419807e-01 -9.9999999997e-01
1.5088972283e-01 -9.9999999997e-01
1.6765524759e-01 -9.9999999998e-01
1.8442077235e-01 -9.9999999998e-01
2.0118629711e-01 -9.9999999998e-01
2.1795182187e-01 -9.9999999998e-01
2.3471734663e-01 -9.9999999999e-01
2.5148287139e-01 -9.9999999999e-01
2.6824839615e-01 -9.9999999999e-01
2.8501392091e-01 -9.9999999999e-01
3.0177944567e-01 -9.9999999999e-01
3.1854497043e-01 -9.9999999999e-01
3.3531049519e-01 -9.9999999999e-01
3.5207601994e-01 -9.9999999999e-01
3.6884154470e-01 -9.9999999999e-01
3.8560706946e-01 -9.9999999999e-01
4.0237259422e-01 -9.9999999999e-01
4.1913811898e-01 -9.9999999999e-01
4.3590364374e-01 -9.9999999999e-01
4.5266916850e-01 -9.9999999999e-01
4.6943469326e-01 -9.9999999999e-01
4.8620021802e-01 -9.9999999999e-01
5.0296574278e-01 -9.9999999999e-01
5.1973126754e-01 -9.9999999999e-01
5.3649679230e-01 -9.9999999999e-01
5.5326231706e-01 -9.9999999999e-01
5.7002784182e-01 -9.9999999999e-01
5.8679336657e-01 -9.9999999999e-01
6.0355889133e-01 -9.9999999999e-01
6.2032441609e-01 -9.9999999998e-01
6.3708994085e-01 -9.9999999998e-01
6.5385546561e-01 -9.9999999998e-01
6.7062099037e-01 -9.9999999998e-01
6.8738651513e-01 -9.9999999997e-01
7.0415203989e-01 -9.9999999997e-01
7.2091756465e-01 -9.9999999996e-01
7.3768308941e-01 -9.9999999995e-01
7.5444861417e-01 -9.9999999994e-01
7.7121413893e-01 -9.9999999992e-01
7.8797966369e-01 -9.9999999987e-01
8.0474518844e-01 -9.9999999976e-01
8.2151071320e-01 -9.9999999880e-01
8.3827623796e-01 9.9999999957e-01
8.5504176272e-01 9.9999999981e-01
8.7180728748e-01 9.9999999988e-01
8.8857281224e-01 9.9999999991e-01
9.0533833700e-01 9.9999999992e-01
9.2210386176e-01 9.9999999993e-01
9.3886938652e-01 9.9999999994e-01
9.5563491128e-01 9.9999999995e-01
9.7240043604e-01 9.9999999995e-01
9.8916596080e-01 9.9999999996e-01
1.0059314856e+00 9.9999999996e-01
1.0226970103e+00 9.9999999996e-01
1.0394625351e+00 9.9999999996e-01
1.0562280598e+00 9.9999999996e-01
1.0729935846e+00 9.9999999996e-01
1.0897591094e+00 9.9999999996e-01
1.1065246341e+00 9.9999999996e-01
1.1232901589e+00 9.9999999996e-01
1.1400556836e+00 9.9999999996e-01
1.1568212084e+00 9.9999999996e-01
1.1735867331e+00 9.9999999996e-01
1.1903522579e+00 9.9999999996e-01
1.2071177827e+00 9.9999999996e-01
1.2238833074e+00 9.9999999996e-01
1.2406488322e+00 9.9999999996e-01
1.2574143569e+00 9.9999999996e-01
1.2741798817e+00 9.9999999996e-01
1.2909454065e+00 9.9999999996e-01
1.3077109312e+00 9.9999999995e-01
1.3244764560e+00 9.9999999995e-01
1.3412419807e+00 9.9999999995e-01
1.3580075055e+00 9.9999999994e-01
1.3747730303e+00 9.9999999994e-01
1.3915385550e+00 9.9999999993e-01
1.4083040798e+00 9.9999999992e-01
1.4250696045e+00 9.9999999991e-01
1.4418351293e+00 9.9999999989e-01
1.4586006541e+00 9.9999999987e-01
1.4753661788e+00 9.9999999983e-01
1.4921317036e+00 9.9999999974e-01
1.5088972283e+00 9.9999999949e-01
1.5256627531e+00 -6.4314085200e-01
1.5424282779e+00 -9.9999999950e-01
1.5591938026e+00 -9.9999999975e-01
1.5759593274e+00 -9.9999999984e-01
1.5927248521e+00 -9.9999999988e-01
1.6094903769e+00 -9.9999999990e-01
1.6262559016e+00 -9.9999999992e-01
1.6430214264e+00 -9.9999999993e-01
1.6597869512e+00 -9.9999999993e-01
1.6765524759e+00 -9.9999999992e-01
1.6933180007e+00 -9.9999999991e-01
1.7100835254e+00 -9.9999999989e-01
1.7268490502e+00 -9.9999999987e-01
1.7436145750e+00 -9.9999999983e-01
1.7603800997e+00 -9.9999999977e-01
1.7771456245e+00 -9.9999999967e-01
1.7939111492e+00 -9.9999999945e-01
1.8106766740e+00 -9.9999999858e-01
1.8274421988e+00 9.9999999649e-01
1.8442077235e+00 9.9999999915e-01
1.8609732483e+00 9.9999999950e-01
1.8777387730e+00 9.9999999963e-01
1.8945042978e+00 9.9999999970e-01
1.9112698226e+00 9.9999999974e-01
1.9280353473e+00 9.9999999977e-01
1.9448008721e+00 9.9999999979e-01
1.9615663968e+00 9.9999999980e-01
1.9783319216e+00 9.9999999981e-01
1.9950974464e+00 9.9999999982e-01
2.0118629711e+00 9.9999999982e-01
2.0286284959e+00 9.9999999983e-01
2.0453940206e+00 9.9999999983e-01
2.0621595454e+00 9.9999999983e-01
2.0789250701e+00 9.9999999983e-01
2.0956905949e+00 9.9999999982e-01
2.1124561197e+00 9.9999999982e-01
2.1292216444e+00 9.9999999981e-01
2.1459871692e+00 9.9999999981e-01
2.1627526939e+00 9.9999999980e-01
2.1795182187e+00 9.9999999979e-01
2.1962837435e+00 9.9999999977e-01
2.2130492682e+00 9.9999999976e-01
2.2298147930e+00 9.9999999974e-01
2.2465803177e+00 9.9999999971e-01
2.2633458425e+00 9.9999999968e-01
2.2801113673e+00 9.9999999965e-01
2.2968768920e+00 9.9999999960e-01
2.3136424168e+00 9.9999999955e-01
2.3304079415e+00 9.9999999948e-01
2.3471734663e+00 9.9999999938e-01
2.3639389911e+00 9.9999999925e-01
2.3807045158e+00 9.9999999906e-01
2.3974700406e+00 9.9999999879e-01
2.4142355653e+00 9.9999999835e-01
2.4310010901e+00 9.9999999760e-01
2.4477666149e+00 9.9999999611e-01
2.4645321396e+00 9.9999999243e-01
2.4812976644e+00 9.9999997788e-01
2.4980631891e+00 1.0155185778e-03
2.5148287139e+00 1.0155185778e-03


==> Figures/Data/s_m2.tex <==
t v
0.0000000000e+00 -2.6587043306e-03
1.6437986647e-02 -1.0999999996e+00
3.2875973294e-02 -1.0999999998e+00
4.9313959940e-02 -1.0999999999e+00
6.5751946587e-02 -1.0999999999e+00
8.2189933234e-02 -1.0999999999e+00
9.8627919881e-02 -1.1000000000e+00
1.1506590653e-01 -1.1000000000e+00
1.3150389317e-01 -1.1000000000e+00
1.4794187982e-01 -1.1000000000e+00
1.6437986647e-01 -1.1000000000e+00
1.8081785312e-01 -1.1000000000e+00
1.9725583976e-01 -1.1000000000e+00
2.1369382641e-01 -1.1000000000e+00
2.3013181306e-01 -1.1000000000e+00
2.4656979970e-01 -1.1000000000e+00
2.6300778635e-01 -1.1000000000e+00
2.7944577300e-01 -1.1000000000e+00
2.9588375964e-01 -1.1000000000e+00
3.1232174629e-01 -1.1000000000e+00
3.2875973294e-01 -1.1000000000e+00
3.4519771958e-01 -1.1000000000e+00
3.6163570623e-01 -1.1000000000e+00
3.7807369288e-01 -1.1000000000e+00
3.9451167952e-01 -1.1000000000e+00
4.1094966617e-01 -1.1000000000e+00
4.2738765282e-01 -1.1000000000e+00
4.4382563946e-01 -1.1000000000e+00
4.6026362611e-01 -1.1000000000e+00
4.7670161276e-01 -1.1000000000e+00
4.9313959940e-01 -1.1000000000e+00
5.0957758605e-01 -1.1000000000e+00
5.2601557270e-01 -1.1000000000e+00
5.4245355935e-01 -1.1000000000e+00
5.5889154599e-01 -1.1000000000e+00
5.7532953264e-01 -1.1000000000e+00
5.9176751929e-01 -1.1000000000e+00
6.0820550593e-01 -1.1000000000e+00
6.2464349258e-01 -1.1000000000e+00
6.4108147923e-01 -1.1000000000e+00
6.5751946587e-01 -1.1000000000e+00
6.7395745252e-01 -1.1000000000e+00
6.9039543917e-01 -1.1000000000e+00
7.0683342581e-01 -1.0999999999e+00
7.2327141246e-01 -1.0999999999e+00
7.3970939911e-01 -1.0999999999e+00
7.5614738575e-01 -1.0999999999e+00
7.7258537240e-01 -1.0999999997e+00
7.8902335905e-01 -1.0999999980e+00
8.0546134569e-01 1.0999999996e+00
8.2189933234e-01 1.0999999998e+00
8.3833731899e-01 1.0999999999e+00
8.5477530564e-01 1.0999999999e+00
8.7121329228e-01 1.0999999999e+00
8.8765127893e-01 1.0999999999e+00
9.0408926558e-01 1.0999999999e+00
9.2052725222e-01 1.0999999999e+00
9.3696523887e-01 1.0999999999e+00
9.5340322552e-01 1.1000000000e+00
9.6984121216e-01 1.1000000000e+00
9.8627919881e-01 1.1000000000e+00
1.0027171855e+00 1.1000000000e+00
1.0191551721e+00 1.1000000000e+00
1.0355931588e+00 1.1000000000e+00
1.0520311454e+00 1.1000000000e+00
1.0684691320e+00 1.1000000000e+00
1.0849071187e+00 1.1000000000e+00
1.1013451053e+00 1.1000000000e+00
1.1177830920e+00 1.1000000000e+00
1.1342210786e+00 1.1000000000e+00
1.1506590653e+00 1.1000000000e+00
1.1670970519e+00 1.1000000000e+00
1.1835350386e+00 1.1000000000e+00
1.1999730252e+00 1.1000000000e+00
1.2164110119e+00 1.1000000000e+00
1.2328489985e+00 1.1000000000e+00
1.2492869852e+00 1.1000000000e+00
1.2657249718e+00 1.0999999999e+00
1.2821629585e+00 1.0999999999e+00
1.2986009451e+00 1.0999999999e+00
1.3150389317e+00 1.0999999999e+00
1.3314769184e+00 1.0999999999e+00
1.3479149050e+00 1.0999999999e+00
1.3643528917e+00 1.0999999999e+00
1.3807908783e+00 1.0999999999e+00
1.3972288650e+00 1.0999999999e+00
1.4136668516e+00 1.0999999999e+00
1.4301048383e+00 1.0999999998e+00
1.4465428249e+00 1.0999999997e+00
1.4629808116e+00 1.0999999994e+00
1.4794187982e+00 7.5927248294e-01
1.4958567849e+00 -1.0999999995e+00
1.5122947715e+00 -1.0999999997e+00
1.5287327582e+00 -1.0999999998e+00
1.5451707448e+00 -1.0999999999e+00
1.5616087314e+00 -1.0999999999e+00
1.5780467181e+00 -1.0999999999e+00
1.5944847047e+00 -1.0999999999e+00
1.6109226914e+00 -1.0999999999e+00
1.6273606780e+00 -1.0999999999e+00
1.6437986647e+00 -1.0999999999e+00
1.6602366513e+00 -1.0999999999e+00
1.6766746380e+00 -1.0999999999e+00
1.6931126246e+00 -1.0999999999e+00
1.7095506113e+00 -1.0999999998e+00
1.7259885979e+00 -1.0999999998e+00
1.7424265846e+00 -1.0999999997e+00
1.7588645712e+00 -1.0999999995e+00
1.7753025579e+00 -1.0999999989e+00
1.7917405445e+00 7.1532710042e-01
1.8081785312e+00 1.0999999988e+00
1.8246165178e+00 1.0999999993e+00
1.8410545044e+00 1.0999999995e+00
1.8574924911e+00 1.0999999996e+00
1.8739304777e+00 1.0999999997e+00
1.8903684644e+00 1.0999999997e+00
1.9068064510e+00 1.0999999998e+00
1.9232444377e+00 1.0999999998e+00
1.9396824243e+00 1.0999999998e+00
1.9561204110e+00 1.0999999998e+00
1.9725583976e+00 1.0999999998e+00
1.9889963843e+00 1.0999999998e+00
2.0054343709e+00 1.0999999998e+00
2.0218723576e+00 1.0999999998e+00
2.0383103442e+00 1.0999999998e+00
2.0547483309e+00 1.0999999998e+00
2.0711863175e+00 1.0999999998e+00
2.0876243041e+00 1.0999999998e+00
2.1040622908e+00 1.0999999998e+00
2.1205002774e+00 1.0999999998e+00
2.1369382641e+00 1.0999999998e+00
2.1533762507e+00 1.0999999997e+00
2.1698142374e+00 1.0999999997e+00
2.1862522240e+00 1.0999999997e+00
2.2026902107e+00 1.0999999997e+00
2.2191281973e+00 1.0999999996e+00
2.2355661840e+00 1.0999999996e+00
2.2520041706e+00 1.0999999995e+00
2.2684421573e+00 1.0999999995e+00
2.2848801439e+00 1.0999999994e+00
2.3013181306e+00 1.0999999993e+00
2.3177561172e+00 1.0999999991e+00
2.3341941038e+00 1.0999999989e+00
2.3506320905e+00 1.0999999986e+00
2.3670700771e+00 1.0999999981e+00
2.3835080638e+00 1.0999999973e+00
2.3999460504e+00 1.0999999956e+00
2.4163840371e+00 1.0999999914e+00
2.4328220237e+00 1.0999999749e+00
2.4492600104e+00 8.3020589586e-05
2.4656979970e+00 8.3020589586e-05


==> Figures/Data/s_m2_approx.tex <==
t v
0.0000000000e+00 -3.2382636614e-02
1.6420657654e-02 -1.0999999996e+00
3.2841315307e-02 -1.0999999998e+00
4.9261972961e-02 -1.0999999999e+00
6.5682630615e-02 -1.0999999999e+00
8.2103288268e-02 -1.0999999999e+00
9.8523945922e-02 -1.1000000000e+00
1.1494460358e-01 -1.1000000000e+00
1.3136526123e-01 -1.1000000000e+00
1.4778591888e-01 -1.1000000000e+00
1.6420657654e-01 -1.1000000000e+00
1.8062723419e-01 -1.1000000000e+00
1.9704789184e-01 -1.1000000000e+00
2.1346854950e-01 -1.1000000000e+00
2.2988920715e-01 -1.1000000000e+00
2.4630986480e-01 -1.1000000000e+00
2.6273052246e-01 -1.1000000000e+00
2.7915118011e-01 -1.1000000000e+00
2.9557183777e-01 -1.1000000000e+00
3.1199249542e-01 -1.1000000000e+00
3.2841315307e-01 -1.1000000000e+00
3.4483381073e-01 -1.1000000000e+00
3.6125446838e-01 -1.1000000000e+00
3.7767512603e-01 -1.1000000000e+00
3.9409578369e-01 -1.1000000000e+00
4.1051644134e-01 -1.1000000000e+00
4.2693709899e-01 -1.1000000000e+00
4.4335775665e-01 -1.1000000000e+00
4.5977841430e-01 -1.1000000000e+00
4.7619907196e-01 -1.1000000000e+00
4.9261972961e-01 -1.1000000000e+00
5.0904038726e-01 -1.1000000000e+00
5.2546104492e-01 -1.1000000000e+00
5.4188170257e-01 -1.1000000000e+00
5.5830236022e-01 -1.1000000000e+00
5.7472301788e-01 -1.1000000000e+00
5.9114367553e-01 -1.1000000000e+00
6.0756433318e-01 -1.1000000000e+00
6.2398499084e-01 -1.1000000000e+00
6.4040564849e-01 -1.1000000000e+00
6.5682630615e-01 -1.1000000000e+00
6.7324696380e-01 -1.1000000000e+00
6.8966762145e-01 -1.1000000000e+00
7.0608827911e-01 -1.1000000000e+00
7.2250893676e-01 -1.1000000000e+00
7.3892959441e-01 -1.0999999999e+00
7.5535025207e-01 -1.0999999999e+00
7.7177090972e-01 -1.0999999999e+00
7.8819156737e-01 -1.0999999998e+00
8.0461222503e-01 -1.0999999988e+00
8.2103288268e-01 1.0999999996e+00
8.3745354034e-01 1.0999999998e+00
8.5387419799e-01 1.0999999999e+00
8.7029485564e-01 1.0999999999e+00
8.8671551330e-01 1.0999999999e+00
9.0313617095e-01 1.0999999999e+00
9.1955682860e-01 1.0999999999e+00
9.3597748626e-01 1.0999999999e+00
9.5239814391e-01 1.1000000000e+00
9.6881880156e-01 1.1000000000e+00
9.8523945922e-01 1.1000000000e+00
1.0016601169e+00 1.1000000000e+00
1.0180807745e+00 1.1000000000e+00
1.0345014322e+00 1.1000000000e+00
1.0509220898e+00 1.1000000000e+00
1.0673427475e+00 1.1000000000e+00
1.0837634051e+00 1.1000000000e+00
1.1001840628e+00 1.1000000000e+00
1.1166047204e+00 1.1000000000e+00
1.1330253781e+00 1.1000000000e+00
1.1494460358e+00 1.1000000000e+00
1.1658666934e+00 1.1000000000e+00
1.1822873511e+00 1.1000000000e+00
1.1987080087e+00 1.1000000000e+00
1.2151286664e+00 1.1000000000e+00
1.2315493240e+00 1.1000000000e+00
1.2479699817e+00 1.1000000000e+00
1.2643906393e+00 1.1000000000e+00
1.2808112970e+00 1.1000000000e+00
1.2972319546e+00 1.1000000000e+00
1.3136526123e+00 1.0999999999e+00
1.3300732699e+00 1.0999999999e+00
1.3464939276e+00 1.0999999999e+00
1.3629145853e+00 1.0999999999e+00
1.3793352429e+00 1.0999999999e+00
1.3957559006e+00 1.0999999999e+00
1.4121765582e+00 1.0999999999e+00
1.4285972159e+00 1.0999999999e+00
1.4450178735e+00 1.0999999998e+00
1.4614385312e+00 1.0999999997e+00
1.4778591888e+00 1.0999999995e+00
1.4942798465e+00 -1.7120277006e+00
1.5107005041e+00 -1.0999999995e+00
1.5271211618e+00 -1.0999999998e+00
1.5435418194e+00 -1.0999999998e+00
1.5599624771e+00 -1.0999999999e+00
1.5763831347e+00 -1.0999999999e+00
1.5928037924e+00 -1.0999999999e+00
1.6092244501e+00 -1.0999999999e+00
1.6256451077e+00 -1.0999999999e+00
1.6420657654e+00 -1.0999999999e+00
1.6584864230e+00 -1.0999999999e+00
1.6749070807e+00 -1.0999999999e+00
1.6913277383e+00 -1.0999999999e+00
1.7077483960e+00 -1.0999999998e+00
1.7241690536e+00 -1.0999999998e+00
1.7405897113e+00 -1.0999999997e+00
1.7570103689e+00 -1.0999999994e+00
1.7734310266e+00 -1.0999999986e+00
1.7898516842e+00 1.0999999965e+00
1.8062723419e+00 1.0999999992e+00
1.8226929996e+00 1.0999999995e+00
1.8391136572e+00 1.0999999996e+00
1.8555343149e+00 1.0999999997e+00
1.8719549725e+00 1.0999999997e+00
1.8883756302e+00 1.0999999998e+00
1.9047962878e+00 1.0999999998e+00
1.9212169455e+00 1.0999999998e+00
1.9376376031e+00 1.0999999998e+00
1.9540582608e+00 1.0999999998e+00
1.9704789184e+00 1.0999999998e+00
1.9868995761e+00 1.0999999998e+00
2.0033202337e+00 1.0999999998e+00
2.0197408914e+00 1.0999999998e+00
2.0361615491e+00 1.0999999998e+00
2.0525822067e+00 1.0999999998e+00
2.0690028644e+00 1.0999999998e+00
2.0854235220e+00 1.0999999998e+00
2.1018441797e+00 1.0999999998e+00
2.1182648373e+00 1.0999999998e+00
2.1346854950e+00 1.0999999998e+00
2.1511061526e+00 1.0999999998e+00
2.1675268103e+00 1.0999999998e+00
2.1839474679e+00 1.0999999997e+00
2.2003681256e+00 1.0999999997e+00
2.2167887832e+00 1.0999999997e+00
2.2332094409e+00 1.0999999996e+00
2.2496300985e+00 1.0999999996e+00
2.2660507562e+00 1.0999999995e+00
2.2824714139e+00 1.0999999995e+00
2.2988920715e+00 1.0999999994e+00
2.3153127292e+00 1.0999999992e+00
2.3317333868e+00 1.0999999991e+00
2.3481540445e+00 1.0999999988e+00
2.3645747021e+00 1.0999999984e+00
2.3809953598e+00 1.0999999976e+00
2.3974160174e+00 1.0999999961e+00
2.4138366751e+00 1.0999999924e+00
2.4302573327e+00 1.0999999779e+00
2.4466779904e+00 1.0111788487e-03
2.4630986480e+00 1.0111788487e-03


==> Figures/Data/x_pos.tex <==
t v
0.0000000000e+00 0.0000000000e+00
1.6765524759e-02 -2.0106356337e-40
3.3531049519e-02 -2.8108282045e-04
5.0296574278e-02 -8.4324846136e-04
6.7062099037e-02 -1.6864969116e-03
8.3827623796e-02 -2.8108280824e-03
1.0059314856e-01 -4.2162416739e-03
1.1735867331e-01 -5.9027369754e-03
1.3412419807e-01 -7.8703125991e-03
1.5088972283e-01 -1.0118966146e-02
1.6765524759e-01 -1.2648693809e-02
1.8442077235e-01 -1.5459489902e-02
2.0118629711e-01 -1.8551346331e-02
2.1795182187e-01 -2.1924251993e-02
2.3471734663e-01 -2.5578192111e-02
2.5148287139e-01 -2.9513147502e-02
2.6824839615e-01 -3.3729093778e-02
2.8501392091e-01 -3.8226000481e-02
3.0177944567e-01 -4.3003830155e-02
3.1854497043e-01 -4.8062537349e-02
3.3531049519e-01 -5.3402067554e-02
3.5207601994e-01 -5.9022356082e-02
3.6884154470e-01 -6.4923326872e-02
3.8560706946e-01 -7.1104891235e-02
4.0237259422e-01 -7.7566946541e-02
4.1913811898e-01 -8.4309374835e-02
4.3590364374e-01 -9.1192910039e-02
4.5266916850e-01 -9.7796359958e-02
4.6943469326e-01 -1.0411989383e-01
4.8620021802e-01 -1.1016368633e-01
5.0296574278e-01 -1.1592791594e-01
5.1973126754e-01 -1.2141276350e-01
5.3649679230e-01 -1.2661841070e-01
5.5326231706e-01 -1.3154503877e-01
5.7002784182e-01 -1.3619282711e-01
5.8679336657e-01 -1.4056195211e-01
6.0355889133e-01 -1.4465258596e-01
6.2032441609e-01 -1.4846489556e-01
6.3708994085e-01 -1.5199904149e-01
6.5385546561e-01 -1.5525517710e-01
6.7062099037e-01 -1.5823344756e-01
6.8738651513e-01 -1.6093398911e-01
7.0415203989e-01 -1.6335692825e-01
7.2091756465e-01 -1.6550238112e-01
7.3768308941e-01 -1.6737045287e-01
7.5444861417e-01 -1.6896123713e-01
7.7121413893e-01 -1.7027481550e-01
7.8797966369e-01 -1.7131125721e-01
8.0474518844e-01 -1.7207061871e-01
8.2151071320e-01 -1.7255294346e-01
8.3827623796e-01 -1.7275826169e-01
8.5504176272e-01 -1.7268659028e-01
8.7180728748e-01 -1.7233793267e-01
8.8857281224e-01 -1.7171229886e-01
9.0533833700e-01 -1.7080971237e-01
9.2210386176e-01 -1.6963021032e-01
9.3886938652e-01 -1.6817384367e-01
9.5563491128e-01 -1.6644067744e-01
9.7240043604e-01 -1.6443079107e-01
9.8916596080e-01 -1.6214427878e-01
1.0059314856e+00 -1.5958125003e-01
1.0226970103e+00 -1.5674183006e-01
1.0394625351e+00 -1.5362616046e-01
1.0562280598e+00 -1.5023439982e-01
1.0729935846e+00 -1.4656672447e-01
1.0897591094e+00 -1.4262332926e-01
1.1065246341e+00 -1.3840442838e-01
1.1232901589e+00 -1.3391025634e-01
1.1400556836e+00 -1.2914106888e-01
1.1568212084e+00 -1.2409714405e-01
1.1735867331e+00 -1.1877878333e-01
1.1903522579e+00 -1.1318631276e-01
1.2071177827e+00 -1.0732008423e-01
1.2238833074e+00 -1.0118047671e-01
1.2406488322e+00 -9.4767897658e-02
1.2574143569e+00 -8.8082784391e-02
1.2741798817e+00 -8.1125605584e-02
1.2909454065e+00 -7.3896862786e-02
1.3077109312e+00 -6.6397091996e-02
1.3244764560e+00 -5.8626865301e-02
1.3412419807e+00 -5.0586792556e-02
1.3580075055e+00 -4.2277523118e-02
1.3747730303e+00 -3.3699747617e-02
1.3915385550e+00 -2.4854199779e-02
1.4083040798e+00 -1.5741658282e-02
1.4250696045e+00 -6.3629486538e-03
1.4418351293e+00 3.2810548025e-03
1.4586006541e+00 1.3189427051e-02
1.4753661788e+00 2.3361190338e-02
1.4921317036e+00 3.3795312195e-02
1.5088972283e+00 4.4490703411e-02
1.5256627531e+00 5.5446216010e-02
1.5424282779e+00 6.6660641207e-02
1.5591938026e+00 7.8132707377e-02
1.5759593274e+00 8.9863255342e-02
1.5927248521e+00 1.0185359427e-01
1.6094903769e+00 1.1410502627e-01
1.6262559016e+00 1.2661884322e-01
1.6430214264e+00 1.3939632347e-01
1.6597869512e+00 1.5243872855e-01
1.6765524759e+00 1.6574729973e-01
1.6933180007e+00 1.7903385584e-01
1.7100835254e+00 1.9205183815e-01
1.7268490502e+00 2.0480011146e-01
1.7436145750e+00 2.1727761516e-01
1.7603800997e+00 2.2948336038e-01
1.7771456245e+00 2.4141642719e-01
1.7939111492e+00 2.5307596173e-01
1.8106766740e+00 2.6446117339e-01
1.8274421988e+00 2.7557133199e-01
1.8442077235e+00 2.8640576493e-01
1.8609732483e+00 2.9696385444e-01
1.8777387730e+00 3.0724620185e-01
1.8945042978e+00 3.1725342899e-01
1.9112698226e+00 3.2698617555e-01
1.9280353473e+00 3.3644509660e-01
1.9448008721e+00 3.4563086009e-01
1.9615663968e+00 3.5454414440e-01
1.9783319216e+00 3.6318563603e-01
1.9950974464e+00 3.7155602727e-01
2.0118629711e+00 3.7965601392e-01
2.0286284959e+00 3.8748629318e-01
2.0453940206e+00 3.9504756150e-01
2.0621595454e+00 4.0234051255e-01
2.0789250701e+00 4.0936583523e-01
2.0956905949e+00 4.1612421177e-01
2.1124561197e+00 4.2261631591e-01
2.1292216444e+00 4.2884281110e-01
2.1459871692e+00 4.3480434882e-01
2.1627526939e+00 4.4050156696e-01
2.1795182187e+00 4.4593508825e-01
2.1962837435e+00 4.5110551877e-01
2.2130492682e+00 4.5601344654e-01
2.2298147930e+00 4.6065944019e-01
2.2465803177e+00 4.6504404763e-01
2.2633458425e+00 4.6916779490e-01
2.2801113673e+00 4.7303118498e-01
2.2968768920e+00 4.7663469675e-01
2.3136424168e+00 4.7997878394e-01
2.3304079415e+00 4.8306387426e-01
2.3471734663e+00 4.8589036845e-01
2.3639389911e+00 4.8845863952e-01
2.3807045158e+00 4.9076903196e-01
2.3974700406e+00 4.9282186113e-01
2.4142355653e+00 4.9461741257e-01
2.4310010901e+00 4.9615594149e-01
2.4477666149e+00 4.9743767226e-01
2.4645321396e+00 4.9846279800e-01
2.4812976644e+00 4.9923148020e-01
2.4980631891e+00 4.9974384841e-01
2.5148287139e+00 5.0000000000e-01


==> Figures/Data/x_pos_m2.tex <==
t v
0.0000000000e+00 0.0000000000e+00
1.6437986647e-02 -8.8107923579e-52
3.2875973294e-02 -2.7020740500e-04
4.9313959940e-02 -8.1062221500e-04
6.5751946587e-02 -1.6212444181e-03
8.2189933234e-02 -2.7020739187e-03
9.8627919881e-02 -4.0531103947e-03
1.1506590653e-01 -5.6743530820e-03
1.3150389317e-01 -7.5658004889e-03
1.4794187982e-01 -9.7274500372e-03
1.6437986647e-01 -1.2159297633e-02
1.8081785312e-01 -1.4861337166e-02
1.9725583976e-01 -1.7833559935e-02
2.1369382641e-01 -2.1075954006e-02
2.3013181306e-01 -2.4588503495e-02
2.4656979970e-01 -2.8371187782e-02
2.6300778635e-01 -3.2423980652e-02
2.7944577300e-01 -3.6746849369e-02
2.9588375964e-01 -4.1339753672e-02
3.1232174629e-01 -4.6202644708e-02
3.2875973294e-01 -5.1335463893e-02
3.4519771958e-01 -5.6738141699e-02
3.6163570623e-01 -6.2410596380e-02
3.7807369288e-01 -6.8352732622e-02
3.9451167952e-01 -7.4564440130e-02
4.1094966617e-01 -8.1045592151e-02
4.2738765282e-01 -8.7369147861e-02
4.4382563946e-01 -9.3423568203e-02
4.6026362611e-01 -9.9209026611e-02
4.7670161276e-01 -1.0472570115e-01
4.9313959940e-01 -1.0997377288e-01
5.0957758605e-01 -1.1495342432e-01
5.2601557270e-01 -1.1966483800e-01
5.4245355935e-01 -1.2410819501e-01
5.5889154599e-01 -1.2828367371e-01
5.7532953264e-01 -1.3219144850e-01
5.9176751929e-01 -1.3583168863e-01
6.0820550593e-01 -1.3920455709e-01
6.2464349258e-01 -1.4231020965e-01
6.4108147923e-01 -1.4514879383e-01
6.5751946587e-01 -1.4772044812e-01
6.7395745252e-01 -1.5002530113e-01
6.9039543917e-01 -1.5206347087e-01
7.0683342581e-01 -1.5383506412e-01
7.2327141246e-01 -1.5534017587e-01
7.3970939911e-01 -1.5657888877e-01
7.5614738575e-01 -1.5755127276e-01
7.7258537240e-01 -1.5825738467e-01
7.8902335905e-01 -1.5869726794e-01
8.0546134569e-01 -1.5887095243e-01
8.2189933234e-01 -1.5877845426e-01
8.3833731899e-01 -1.5841977575e-01
8.5477530564e-01 -1.5779492840e-01
8.7121329228e-01 -1.5690393763e-01
8.8765127893e-01 -1.5574684285e-01
9.0408926558e-01 -1.5432369775e-01
9.2052725222e-01 -1.5263457053e-01
9.3696523887e-01 -1.5067954428e-01
9.5340322552e-01 -1.4845871738e-01
9.6984121216e-01 -1.4597220402e-01
9.8627919881e-01 -1.4322013476e-01
1.0027171855e+00 -1.4020265717e-01
1.0191551721e+00 -1.3691993652e-01
1.0355931588e+00 -1.3337215660e-01
1.0520311454e+00 -1.2955952052e-01
1.0684691320e+00 -1.2548225167e-01
1.0849071187e+00 -1.2114059469e-01
1.1013451053e+00 -1.1653481655e-01
1.1177830920e+00 -1.1166520764e-01
1.1342210786e+00 -1.0653208300e-01
1.1506590653e+00 -1.0113578357e-01
1.1670970519e+00 -9.5476677522e-02
1.1835350386e+00 -8.9555161637e-02
1.1999730252e+00 -8.3371662790e-02
1.2164110119e+00 -7.6926639446e-02
1.2328489985e+00 -7.0220583253e-02
1.2492869852e+00 -6.3254020673e-02
1.2657249718e+00 -5.6027514681e-02
1.2821629585e+00 -4.8541666512e-02
1.2986009451e+00 -4.0797117465e-02
1.3150389317e+00 -3.2794550753e-02
1.3314769184e+00 -2.4534693396e-02
1.3479149050e+00 -1.6018318167e-02
1.3643528917e+00 -7.2462455669e-03
1.3807908783e+00 1.7806541606e-03
1.3972288650e+00 1.1061458983e-02
1.4136668516e+00 2.0595193006e-02
1.4301048383e+00 3.0380824380e-02
1.4465428249e+00 4.0417263190e-02
1.4629808116e+00 5.0703359329e-02
1.4794187982e+00 6.1237900375e-02
1.4958567849e+00 7.2019609458e-02
1.5122947715e+00 8.3047143146e-02
1.5287327582e+00 9.4319530774e-02
1.5451707448e+00 1.0583820444e-01
1.5616087314e+00 1.1760459046e-01
1.5780467181e+00 1.2962010591e-01
1.5944847047e+00 1.4188615507e-01
1.6109226914e+00 1.5440412577e-01
1.6273606780e+00 1.6717538562e-01
1.6437986647e+00 1.8015815897e-01
1.6602366513e+00 1.9288498397e-01
1.6766746380e+00 2.0535458108e-01
1.6931126246e+00 2.1756575319e-01
1.7095506113e+00 2.2951738269e-01
1.7259885979e+00 2.4120842845e-01
1.7424265846e+00 2.5263792288e-01
1.7588645712e+00 2.6380496885e-01
1.7753025579e+00 2.7470873671e-01
1.7917405445e+00 2.8534846122e-01
1.8081785312e+00 2.9572343857e-01
1.8246165178e+00 3.0583302339e-01
1.8410545044e+00 3.1567761977e-01
1.8574924911e+00 3.2525786477e-01
1.8739304777e+00 3.3457441538e-01
1.8903684644e+00 3.4362794582e-01
1.9068064510e+00 3.5241914491e-01
1.9232444377e+00 3.6094871344e-01
1.9396824243e+00 3.6921736168e-01
1.9561204110e+00 3.7722580683e-01
1.9725583976e+00 3.8497477068e-01
1.9889963843e+00 3.9246497727e-01
2.0054343709e+00 3.9969715058e-01
2.0218723576e+00 4.0667201237e-01
2.0383103442e+00 4.1339028004e-01
2.0547483309e+00 4.1985266458e-01
2.0711863175e+00 4.2605986862e-01
2.0876243041e+00 4.3201258450e-01
2.1040622908e+00 4.3771149246e-01
2.1205002774e+00 4.4315725889e-01
2.1369382641e+00 4.4835053466e-01
2.1533762507e+00 4.5329195352e-01
2.1698142374e+00 4.5798213057e-01
2.1862522240e+00 4.6242166084e-01
2.2026902107e+00 4.6661111788e-01
2.2191281973e+00 4.7055105251e-01
2.2355661840e+00 4.7424199155e-01
2.2520041706e+00 4.7768443667e-01
2.2684421573e+00 4.8087886337e-01
2.2848801439e+00 4.8382571989e-01
2.3013181306e+00 4.8652542635e-01
2.3177561172e+00 4.8897837381e-01
2.3341941038e+00 4.9118492353e-01
2.3506320905e+00 4.9314540624e-01
2.3670700771e+00 4.9486012143e-01
2.3835080638e+00 4.9632933681e-01
2.3999460504e+00 4.9755328776e-01
2.4163840371e+00 4.9853217690e-01
2.4328220237e+00 4.9926617365e-01
2.4492600104e+00 4.9975541396e-01
2.4656979970e+00 5.0000000000e-01


==> Figures/Data/x_pos_m2_approx.tex <==
t v
0.0000000000e+00 0.0000000000e+00
1.6420657654e-02 -1.9692768384e-40
3.2841315307e-02 -2.6951906446e-04
4.9261972961e-02 -8.0855719337e-04
6.5682630615e-02 -1.6171143748e-03
8.2103288268e-02 -2.6951905131e-03
9.8523945922e-02 -4.0427852854e-03
1.1494460358e-01 -5.6598979269e-03
1.3136526123e-01 -7.5465269431e-03
1.4778591888e-01 -9.7026697520e-03
1.6420657654e-01 -1.2128322253e-02
1.8062723419e-01 -1.4823478327e-02
1.9704789184e-01 -1.7788129259e-02
2.1346854950e-01 -2.1022263097e-02
2.2988920715e-01 -2.4525863931e-02
2.4630986480e-01 -2.8298911111e-02
2.6273052246e-01 -3.2341378380e-02
2.7915118011e-01 -3.6653232951e-02
2.9557183777e-01 -4.1234434501e-02
3.1199249542e-01 -4.6084934102e-02
3.2841315307e-01 -5.1204673076e-02
3.4483381073e-01 -5.6593581790e-02
3.6125446838e-01 -6.2251578368e-02
3.7767512603e-01 -6.8178567348e-02
3.9409578369e-01 -7.4374438264e-02
4.1051644134e-01 -8.0839064160e-02
4.2693709899e-01 -8.7128128158e-02
4.4335775665e-01 -9.3148746805e-02
4.5977841430e-01 -9.8901094249e-02
4.7619907196e-01 -1.0438534931e-01
4.9261972961e-01 -1.0960169384e-01
5.0904038726e-01 -1.1455031119e-01
5.2546104492e-01 -1.1923138472e-01
5.4188170257e-01 -1.2364509639e-01
5.5830236022e-01 -1.2779162544e-01
5.7472301788e-01 -1.3167114715e-01
5.9114367553e-01 -1.3528383164e-01
6.0756433318e-01 -1.3862984278e-01
6.2398499084e-01 -1.4170933717e-01
6.4040564849e-01 -1.4452246320e-01
6.5682630615e-01 -1.4706936014e-01
6.7324696380e-01 -1.4935015738e-01
6.8966762145e-01 -1.5136497369e-01
7.0608827911e-01 -1.5311391654e-01
7.2250893676e-01 -1.5459708157e-01
7.3892959441e-01 -1.5581455206e-01
7.5535025207e-01 -1.5676639846e-01
7.7177090972e-01 -1.5745267811e-01
7.8819156737e-01 -1.5787343487e-01
8.0461222503e-01 -1.5802869897e-01
8.2103288268e-01 -1.5791848679e-01
8.3745354034e-01 -1.5754280087e-01
8.5387419799e-01 -1.5690162982e-01
8.7029485564e-01 -1.5599499889e-01
8.8671551330e-01 -1.5482294734e-01
9.0313617095e-01 -1.5338552864e-01
9.1955682860e-01 -1.5168281079e-01
9.3597748626e-01 -1.4971487661e-01
9.5239814391e-01 -1.4748182422e-01
9.6881880156e-01 -1.4498376749e-01
9.8523945922e-01 -1.4222083662e-01
1.0016601169e+00 -1.3919317880e-01
1.0180807745e+00 -1.3590095885e-01
1.0345014322e+00 -1.3234436008e-01
1.0509220898e+00 -1.2852358508e-01
1.0673427475e+00 -1.2443885665e-01
1.0837634051e+00 -1.2009041880e-01
1.1001840628e+00 -1.1547853779e-01
1.1166047204e+00 -1.1060350328e-01
1.1330253781e+00 -1.0546562950e-01
1.1494460358e+00 -1.0006525652e-01
1.1658666934e+00 -9.4402751590e-02
1.1822873511e+00 -8.8478510513e-02
1.1987080087e+00 -8.2292959116e-02
1.2151286664e+00 -7.5846554765e-02
1.2315493240e+00 -6.9139787947e-02
1.2479699817e+00 -6.2173183910e-02
1.2643906393e+00 -5.4947304360e-02
1.2808112970e+00 -4.7462749215e-02
1.2972319546e+00 -3.9720158407e-02
1.3136526123e+00 -3.1720213742e-02
1.3300732699e+00 -2.3463640797e-02
1.3464939276e+00 -1.4951210871e-02
1.3629145853e+00 -6.1837429650e-03
1.3793352429e+00 2.8378941895e-03
1.3957559006e+00 1.2112780080e-02
1.4121765582e+00 2.1639940327e-02
1.4285972159e+00 3.1418344582e-02
1.4450178735e+00 4.1446904399e-02
1.4614385312e+00 5.1724471099e-02
1.4778591888e+00 6.2249833631e-02
1.4942798465e+00 7.3021716419e-02
1.5107005041e+00 8.4038777230e-02
1.5271211618e+00 9.5299605045e-02
1.5435418194e+00 1.0680643396e-01
1.5599624771e+00 1.1856067950e-01
1.5763831347e+00 1.3056374752e-01
1.5928037924e+00 1.4281703067e-01
1.6092244501e+00 1.5532190474e-01
1.6256451077e+00 1.6807972493e-01
1.6420657654e+00 1.8109182203e-01
1.6584864230e+00 1.9378475477e-01
1.6749070807e+00 2.0622083794e-01
1.6913277383e+00 2.1839888749e-01
1.7077483960e+00 2.3031779882e-01
1.7241690536e+00 2.4197654372e-01
1.7405897113e+00 2.5337416738e-01
1.7570103689e+00 2.6450978533e-01
1.7734310266e+00 2.7538258041e-01
1.7898516842e+00 2.8599179968e-01
1.8062723419e+00 2.9633675145e-01
1.8226929996e+00 3.0641680224e-01
1.8391136572e+00 3.1623256850e-01
1.8555343149e+00 3.2578468942e-01
1.8719549725e+00 3.3507382412e-01
1.8883756302e+00 3.4410064897e-01
1.9047962878e+00 3.5286585493e-01
1.9212169455e+00 3.6137014492e-01
1.9376376031e+00 3.6961423130e-01
1.9540582608e+00 3.7759883340e-01
1.9704789184e+00 3.8532467508e-01
1.9868995761e+00 3.9279248241e-01
2.0033202337e+00 4.0000298141e-01
2.0197408914e+00 4.0695689583e-01
2.0361615491e+00 4.1365494501e-01
2.0525822067e+00 4.2009784188e-01
2.0690028644e+00 4.2628629092e-01
2.0854235220e+00 4.3222098630e-01
2.1018441797e+00 4.3790261006e-01
2.1182648373e+00 4.4333183030e-01
2.1346854950e+00 4.4850929958e-01
2.1511061526e+00 4.5343565327e-01
2.1675268103e+00 4.5811150804e-01
2.1839474679e+00 4.6253746042e-01
2.2003681256e+00 4.6671408541e-01
2.2167887832e+00 4.7064193520e-01
2.2332094409e+00 4.7432153793e-01
2.2496300985e+00 4.7775339654e-01
2.2660507562e+00 4.8093798767e-01
2.2824714139e+00 4.8387576069e-01
2.2988920715e+00 4.8656713674e-01
2.3153127292e+00 4.8901250786e-01
2.3317333868e+00 4.9121223619e-01
2.3481540445e+00 4.9316665325e-01
2.3645747021e+00 4.9487605927e-01
2.3809953598e+00 4.9634072263e-01
2.3974160174e+00 4.9756087927e-01
2.4138366751e+00 4.9853673230e-01
2.4302573327e+00 4.9926845156e-01
2.4466779904e+00 4.9975617332e-01
2.4630986480e+00 5.0000000000e-01


==> Figures/Data/y_pos.tex <==
t v
0.0000000000e+00 0.0000000000e+00
1.6765524759e-02 -1.9382836737e-47
3.3531049519e-02 -1.9382836737e-47
5.0296574278e-02 -1.4184964248e-43
6.7062099037e-02 -7.9007550884e-08
8.3827623796e-02 -3.9503772324e-07
1.0059314856e-01 -1.1851129076e-06
1.1735867331e-01 -2.7652621653e-06
1.3412419807e-01 -5.5305197053e-06
1.5088972283e-01 -9.9549219193e-06
1.6765524759e-01 -1.6591502263e-05
1.8442077235e-01 -2.6072283131e-05
2.0118629711e-01 -3.9108263719e-05
2.1795182187e-01 -5.6489402750e-05
2.3471734663e-01 -7.9084594753e-05
2.5148287139e-01 -1.0784163850e-04
2.6824839615e-01 -1.4378719599e-04
2.8501392091e-01 -1.8802674034e-04
3.0177944567e-01 -2.4174449067e-04
3.1854497043e-01 -3.0620333195e-04
3.3531049519e-01 -3.8274471791e-04
3.5207601994e-01 -4.7278855444e-04
3.6884154470e-01 -5.7783306129e-04
3.8560706946e-01 -6.9945460956e-04
4.0237259422e-01 -8.3930753223e-04
4.1913811898e-01 -9.9912390497e-04
4.3590364374e-01 -1.1699035309e-03
4.5266916850e-01 -1.3170233696e-03
4.6943469326e-01 -1.4385588342e-03
4.8620021802e-01 -1.5326660063e-03
5.0296574278e-01 -1.5975816133e-03
5.1973126754e-01 -1.6316229785e-03
5.3649679230e-01 -1.6331879488e-03
5.5326231706e-01 -1.6007548006e-03
5.7002784182e-01 -1.5328821304e-03
5.8679336657e-01 -1.4282087293e-03
6.0355889133e-01 -1.2854534475e-03
6.2032441609e-01 -1.1034150488e-03
6.3708994085e-01 -8.8097205928e-04
6.5385546561e-01 -6.1708261080e-04
6.7062099037e-01 -3.1078428336e-04
6.8738651513e-01 3.8806053450e-05
7.0415203989e-01 4.3249239720e-04
7.2091756465e-01 8.7099976612e-04
7.3768308941e-01 1.3549743480e-03
7.5444861417e-01 1.8849836431e-03
7.7121413893e-01 2.4615165993e-03
7.8797966369e-01 3.0849837402e-03
8.0474518844e-01 3.7557172826e-03
8.2151071320e-01 4.4739712454e-03
8.3827623796e-01 5.2399215469e-03
8.5504176272e-01 6.0536660925e-03
8.7180728748e-01 6.9152248500e-03
8.8857281224e-01 7.8246557224e-03
9.0533833700e-01 8.7820945051e-03
9.2210386176e-01 9.7877549271e-03
9.3886938652e-01 1.0841928681e-02
9.5563491128e-01 1.1944985441e-02
9.7240043604e-01 1.3097372867e-02
9.8916596080e-01 1.4299616599e-02
1.0059314856e+00 1.5552320230e-02
1.0226970103e+00 1.6856165273e-02
1.0394625351e+00 1.8211911105e-02
1.0562280598e+00 1.9620394893e-02
1.0729935846e+00 2.1082531508e-02
1.0897591094e+00 2.2599313410e-02
1.1065246341e+00 2.4171810516e-02
1.1232901589e+00 2.5801170041e-02
1.1400556836e+00 2.7488616315e-02
1.1568212084e+00 2.9235450572e-02
1.1735867331e+00 3.1043050703e-02
1.1903522579e+00 3.2912870985e-02
1.2071177827e+00 3.4846441770e-02
1.2238833074e+00 3.6845369132e-02
1.2406488322e+00 3.8911334479e-02
1.2574143569e+00 4.1046094123e-02
1.2741798817e+00 4.3251478794e-02
1.2909454065e+00 4.5529393115e-02
1.3077109312e+00 4.7881815018e-02
1.3244764560e+00 5.0310795104e-02
1.3412419807e+00 5.2818455948e-02
1.3580075055e+00 5.5406991336e-02
1.3747730303e+00 5.8078665441e-02
1.3915385550e+00 6.0835811923e-02
1.4083040798e+00 6.3680832966e-02
1.4250696045e+00 6.6616198227e-02
1.4418351293e+00 6.9644443716e-02
1.4586006541e+00 7.2768170584e-02
1.4753661788e+00 7.5990043834e-02
1.4921317036e+00 7.9312790932e-02
1.5088972283e+00 8.2739200336e-02
1.5256627531e+00 8.6272119919e-02
1.5424282779e+00 8.9914455307e-02
1.5591938026e+00 9.3669168099e-02
1.5759593274e+00 9.7534310570e-02
1.5927248521e+00 1.0150676663e-01
1.6094903769e+00 1.0558332821e-01
1.6262559016e+00 1.0976069502e-01
1.6430214264e+00 1.1403547442e-01
1.6597869512e+00 1.1840418137e-01
1.6765524759e+00 1.2286323853e-01
1.6933180007e+00 1.2731515882e-01
1.7100835254e+00 1.3168415946e-01
1.7268490502e+00 1.3597401081e-01
1.7436145750e+00 1.4018842101e-01
1.7603800997e+00 1.4433103370e-01
1.7771456245e+00 1.4840542591e-01
1.7939111492e+00 1.5241510607e-01
1.8106766740e+00 1.5636351215e-01
1.8274421988e+00 1.6025401000e-01
1.8442077235e+00 1.6408989180e-01
1.8609732483e+00 1.6787437457e-01
1.8777387730e+00 1.7160432432e-01
1.8945042978e+00 1.7527668602e-01
1.9112698226e+00 1.7888848397e-01
1.9280353473e+00 1.8243682217e-01
1.9448008721e+00 1.8591888446e-01
1.9615663968e+00 1.8933193477e-01
1.9783319216e+00 1.9267331716e-01
1.9950974464e+00 1.9594045588e-01
2.0118629711e+00 1.9913085532e-01
2.0286284959e+00 2.0224210001e-01
2.0453940206e+00 2.0527185441e-01
2.0621595454e+00 2.0821786281e-01
2.0789250701e+00 2.1107794910e-01
2.0956905949e+00 2.1385001658e-01
2.1124561197e+00 2.1653204763e-01
2.1292216444e+00 2.1912210348e-01
2.1459871692e+00 2.2161832387e-01
2.1627526939e+00 2.2401892674e-01
2.1795182187e+00 2.2632220787e-01
2.1962837435e+00 2.2852654052e-01
2.2130492682e+00 2.3063037511e-01
2.2298147930e+00 2.3263223880e-01
2.2465803177e+00 2.3453073516e-01
2.2633458425e+00 2.3632454379e-01
2.2801113673e+00 2.3801241995e-01
2.2968768920e+00 2.3959319424e-01
2.3136424168e+00 2.4106577220e-01
2.3304079415e+00 2.4242913399e-01
2.3471734663e+00 2.4368233412e-01
2.3639389911e+00 2.4482450106e-01
2.3807045158e+00 2.4585483701e-01
2.3974700406e+00 2.4677261760e-01
2.4142355653e+00 2.4757719163e-01
2.4310010901e+00 2.4826798089e-01
2.4477666149e+00 2.4884447988e-01
2.4645321396e+00 2.4930625569e-01
2.4812976644e+00 2.4965294779e-01
2.4980631891e+00 2.4988426792e-01
2.5148287139e+00 2.5000000000e-01


==> Figures/Data/y_pos_m2.tex <==
t v
0.0000000000e+00 0.0000000000e+00
1.6437986647e-02 0.0000000000e+00
3.2875973294e-02 2.5030830779e-71
4.9313959940e-02 -2.0189466900e-47
6.5751946587e-02 -8.0313244677e-08
8.2189933234e-02 -4.0156618794e-07
9.8627919881e-02 -1.2046982659e-06
1.1506590653e-01 -2.8109611589e-06
1.3150389317e-01 -5.6219170603e-06
1.4794187982e-01 -1.0119435307e-05
1.6437986647e-01 -1.6865686559e-05
1.8081785312e-01 -2.6503133567e-05
1.9725583976e-01 -3.9754517375e-05
2.1369382641e-01 -5.7422837685e-05
2.3013181306e-01 -8.0391325896e-05
2.4656979970e-01 -1.0962340923e-04
2.6300778635e-01 -1.4616266411e-04
2.7944577300e-01 -1.9113275696e-04
2.9588375964e-01 -2.4573737014e-04
3.1232174629e-01 -3.1126011094e-04
3.2875973294e-01 -3.8906440118e-04
3.4519771958e-01 -4.8059334474e-04
3.6163570623e-01 -5.8736957043e-04
3.7807369288e-01 -7.1099504736e-04
3.9451167952e-01 -8.5315086965e-04
4.1094966617e-01 -1.0155970075e-03
4.2738765282e-01 -1.1650931547e-03
4.4382563946e-01 -1.2905436013e-03
4.6026362611e-01 -1.3900803490e-03
4.7670161276e-01 -1.4619174301e-03
4.9313959940e-01 -1.5043508661e-03
5.0957758605e-01 -1.5157585994e-03
5.2601557270e-01 -1.4946004018e-03
5.4245355935e-01 -1.4394177632e-03
5.5889154599e-01 -1.3488337634e-03
5.7532953264e-01 -1.2215529312e-03
5.9176751929e-01 -1.0563610920e-03
6.0820550593e-01 -8.5212520817e-04
6.2464349258e-01 -6.0779321439e-04
6.4108147923e-01 -3.2239384953e-04
6.5751946587e-01 4.9635117013e-06
6.7395745252e-01 3.7508902577e-04
6.9039543917e-01 7.8871254421e-04
7.0683342581e-01 1.2464837725e-03
7.2327141246e-01 1.7489724224e-03
7.3970939911e-01 2.2966683571e-03
7.5614738575e-01 2.8899817267e-03
7.7258537240e-01 3.5292430940e-03
7.8902335905e-01 4.2147035502e-03
8.0546134569e-01 4.9465348184e-03
8.2189933234e-01 5.7248293459e-03
8.3833731899e-01 6.5496003836e-03
8.5477530564e-01 7.4209138064e-03
8.7121329228e-01 8.3389146481e-03
8.8765127893e-01 9.3038271440e-03
9.0408926558e-01 1.0315954761e-02
9.2052725222e-01 1.1375680213e-02
9.3696523887e-01 1.2483465466e-02
9.5340322552e-01 1.3639851723e-02
9.6984121216e-01 1.4845459398e-02
9.8627919881e-01 1.6100988071e-02
1.0027171855e+00 1.7407216427e-02
1.0191551721e+00 1.8765002170e-02
1.0355931588e+00 2.0175281922e-02
1.0520311454e+00 2.1639071095e-02
1.0684691320e+00 2.3157463742e-02
1.0849071187e+00 2.4731632376e-02
1.1013451053e+00 2.6362827762e-02
1.1177830920e+00 2.8052378678e-02
1.1342210786e+00 2.9801691641e-02
1.1506590653e+00 3.1612250596e-02
1.1670970519e+00 3.3485616563e-02
1.1835350386e+00 3.5423427247e-02
1.1999730252e+00 3.7427396593e-02
1.2164110119e+00 3.9499314301e-02
1.2328489985e+00 4.1641045284e-02
1.2492869852e+00 4.3854529064e-02
1.2657249718e+00 4.6141779125e-02
1.2821629585e+00 4.8504882183e-02
1.2986009451e+00 5.0945997403e-02
1.3150389317e+00 5.3467355539e-02
1.3314769184e+00 5.6071258005e-02
1.3479149050e+00 5.8760075859e-02
1.3643528917e+00 6.1536248713e-02
1.3807908783e+00 6.4402283554e-02
1.3972288650e+00 6.7360753479e-02
1.4136668516e+00 7.0414296328e-02
1.4301048383e+00 7.3565613234e-02
1.4465428249e+00 7.6817467059e-02
1.4629808116e+00 8.0172680739e-02
1.4794187982e+00 8.3634135513e-02
1.4958567849e+00 8.7204769053e-02
1.5122947715e+00 9.0887573470e-02
1.5287327582e+00 9.4684652071e-02
1.5451707448e+00 9.8592884758e-02
1.5616087314e+00 1.0260905554e-01
1.5780467181e+00 1.0672985216e-01
1.5944847047e+00 1.1095186587e-01
1.6109226914e+00 1.1527159131e-01
1.6273606780e+00 1.1968542652e-01
1.6437986647e+00 1.2417436296e-01
1.6602366513e+00 1.2857668251e-01
1.6766746380e+00 1.3289626238e-01
1.6931126246e+00 1.3713692100e-01
1.7095506113e+00 1.4130241534e-01
1.7259885979e+00 1.4539643828e-01
1.7424265846e+00 1.4942261624e-01
1.7588645712e+00 1.5338450695e-01
1.7753025579e+00 1.5728559738e-01
1.7917405445e+00 1.6112930182e-01
1.8081785312e+00 1.6491896013e-01
1.8246165178e+00 1.6865783610e-01
1.8410545044e+00 1.7234386160e-01
1.8574924911e+00 1.7597393724e-01
1.8739304777e+00 1.7954504418e-01
1.8903684644e+00 1.8305424446e-01
1.9068064510e+00 1.8649868129e-01
1.9232444377e+00 1.8987557927e-01
1.9396824243e+00 1.9318224453e-01
1.9561204110e+00 1.9641606477e-01
1.9725583976e+00 1.9957450927e-01
1.9889963843e+00 2.0265512885e-01
2.0054343709e+00 2.0565555573e-01
2.0218723576e+00 2.0857350340e-01
2.0383103442e+00 2.1140676636e-01
2.0547483309e+00 2.1415321994e-01
2.0711863175e+00 2.1681081998e-01
2.0876243041e+00 2.1937760251e-01
2.1040622908e+00 2.2185168348e-01
2.1205002774e+00 2.2423125832e-01
2.1369382641e+00 2.2651460163e-01
2.1533762507e+00 2.2870006676e-01
2.1698142374e+00 2.3078608544e-01
2.1862522240e+00 2.3277116734e-01
2.2026902107e+00 2.3465389972e-01
2.2191281973e+00 2.3643294698e-01
2.2355661840e+00 2.3810705028e-01
2.2520041706e+00 2.3967502714e-01
2.2684421573e+00 2.4113577108e-01
2.2848801439e+00 2.4248825121e-01
2.3013181306e+00 2.4373151191e-01
2.3177561172e+00 2.4486467247e-01
2.3341941038e+00 2.4588692677e-01
2.3506320905e+00 2.4679754298e-01
2.3670700771e+00 2.4759586329e-01
2.3835080638e+00 2.4828130364e-01
2.3999460504e+00 2.4885335350e-01
2.4163840371e+00 2.4931157564e-01
2.4328220237e+00 2.4965560601e-01
2.4492600104e+00 2.4988515353e-01
2.4656979970e+00 2.5000000000e-01


==> Figures/Data/y_pos_m2_approx.tex <==
t v
0.0000000000e+00 0.0000000000e+00
1.6420657654e-02 -8.5205711095e-24
3.2841315307e-02 -1.7041141546e-23
4.9261972961e-02 -2.5561711982e-23
6.5682630615e-02 -8.0407559639e-08
8.2103288268e-02 -4.0203776279e-07
9.8523945922e-02 -1.2061129907e-06
1.1494460358e-01 -2.8142621851e-06
1.3136526123e-01 -5.6285191184e-06
1.4778591888e-01 -1.0131319028e-05
1.6420657654e-01 -1.6885492803e-05
1.8062723419e-01 -2.6534257758e-05
1.9704789184e-01 -3.9801203859e-05
2.1346854950e-01 -5.7490274095e-05
2.2988920715e-01 -8.0485737563e-05
2.4630986480e-01 -1.0975215361e-04
2.6273052246e-01 -1.4633432531e-04
2.7915118011e-01 -1.9135724023e-04
2.9557183777e-01 -2.4602599655e-04
3.1199249542e-01 -3.1162571210e-04
3.2841315307e-01 -3.8952141407e-04
3.4483381073e-01 -4.8115790670e-04
3.6125446838e-01 -5.8805961429e-04
3.7767512603e-01 -7.1183039676e-04
3.9409578369e-01 -8.5415333460e-04
4.1051644134e-01 -1.0167904802e-03
4.2693709899e-01 -1.1664346270e-03
4.4335775665e-01 -1.2920047283e-03
4.5977841430e-01 -1.3916306903e-03
4.7619907196e-01 -1.4635245567e-03
4.9261972961e-01 -1.5059804676e-03
5.0904038726e-01 -1.5173745917e-03
5.2546104492e-01 -1.4961650348e-03
5.4188170257e-01 -1.4408917285e-03
5.5830236022e-01 -1.3501763014e-03
5.7472301788e-01 -1.2227219381e-03
5.9114367553e-01 -1.0573132256e-03
6.0756433318e-01 -8.5281599349e-04
6.2398499084e-01 -6.0817714740e-04
6.4040564849e-01 -3.2242450051e-04
6.5682630615e-01 5.3333963207e-06
6.7324696380e-01 3.7590742292e-04
6.8966762145e-01 7.9002805496e-04
7.0608827911e-01 1.2483455243e-03
7.2250893676e-01 1.7514299731e-03
7.3892959441e-01 2.2997715998e-03
7.5535025207e-01 2.8937807966e-03
7.7177090972e-01 3.5337882769e-03
7.8819156737e-01 4.2200451919e-03
8.0461222503e-01 4.9527232358e-03
8.2103288268e-01 5.7319147395e-03
8.3745354034e-01 6.5576327511e-03
8.5387419799e-01 7.4298111049e-03
8.7029485564e-01 8.3485951159e-03
8.8671551330e-01 9.3142093966e-03
9.0313617095e-01 1.0326957889e-02
9.1955682860e-01 1.1387223880e-02
9.3597748626e-01 1.2495470010e-02
9.5239814391e-01 1.3652238259e-02
9.6881880156e-01 1.4858149920e-02
9.8523945922e-01 1.6113905559e-02
1.0016601169e+00 1.7420284954e-02
1.0180807745e+00 1.8778147015e-02
1.0345014322e+00 2.0188429681e-02
1.0509220898e+00 2.1652149799e-02
1.0673427475e+00 2.3170402976e-02
1.0837634051e+00 2.4744363401e-02
1.1001840628e+00 2.6375283645e-02
1.1166047204e+00 2.8064494420e-02
1.1330253781e+00 2.9813404317e-02
1.1494460358e+00 3.1623499492e-02
1.1658666934e+00 3.3496343326e-02
1.1822873511e+00 3.5433576034e-02
1.1987080087e+00 3.7436914232e-02
1.2151286664e+00 3.9508150455e-02
1.2315493240e+00 4.1649152622e-02
1.2479699817e+00 4.3861863444e-02
1.2643906393e+00 4.6148299776e-02
1.2808112970e+00 4.8510551904e-02
1.2972319546e+00 5.0950782768e-02
1.3136526123e+00 5.3471227107e-02
1.3300732699e+00 5.6074190545e-02
1.3464939276e+00 5.8762048582e-02
1.3629145853e+00 6.1537245513e-02
1.3793352429e+00 6.4402293263e-02
1.3957559006e+00 6.7359770126e-02
1.4121765582e+00 7.0412319419e-02
1.4285972159e+00 7.3562648029e-02
1.4450178735e+00 7.6813524873e-02
1.4614385312e+00 8.0167779244e-02
1.4778591888e+00 8.3628299058e-02
1.4942798465e+00 8.7198028985e-02
1.5107005041e+00 9.0879968477e-02
1.5271211618e+00 9.4677169670e-02
1.5435418194e+00 9.8584580115e-02
1.5599624771e+00 1.0259897213e-01
1.5763831347e+00 1.0671702198e-01
1.5928037924e+00 1.1093530965e-01
1.6092244501e+00 1.1525031874e-01
1.6256451077e+00 1.1965843650e-01
1.6420657654e+00 1.2415595403e-01
1.6584864230e+00 1.2854977874e-01
1.6749070807e+00 1.3286190854e-01
1.6913277383e+00 1.3709617039e-01
1.7077483960e+00 1.4125632917e-01
1.7241690536e+00 1.4534608512e-01
1.7405897113e+00 1.4936907149e-01
1.7570103689e+00 1.5332885228e-01
1.7734310266e+00 1.5722892021e-01
1.7898516842e+00 1.6107269482e-01
1.8062723419e+00 1.6486352074e-01
1.8226929996e+00 1.6860466608e-01
1.8391136572e+00 1.7229294784e-01
1.8555343149e+00 1.7592526319e-01
1.8719549725e+00 1.7949858993e-01
1.8883756302e+00 1.8300998686e-01
1.9047962878e+00 1.8645659406e-01
1.9212169455e+00 1.8983563310e-01
1.9376376031e+00 1.9314440720e-01
1.9540582608e+00 1.9638030122e-01
1.9704789184e+00 1.9954078174e-01
1.9868995761e+00 2.0262339696e-01
2.0033202337e+00 2.0562577658e-01
2.0197408914e+00 2.0854563163e-01
2.0361615491e+00 2.1138075430e-01
2.0525822067e+00 2.1412901767e-01
2.0690028644e+00 2.1678837541e-01
2.0854235220e+00 2.1935686152e-01
2.1018441797e+00 2.2183258994e-01
2.1182648373e+00 2.2421375422e-01
2.1346854950e+00 2.2649862715e-01
2.1511061526e+00 2.2868556037e-01
2.1675268103e+00 2.3077298396e-01
2.1839474679e+00 2.3275940605e-01
2.2003681256e+00 2.3464341240e-01
2.2167887832e+00 2.3642366605e-01
2.2332094409e+00 2.3809890682e-01
2.2496300985e+00 2.3966795103e-01
2.2660507562e+00 2.4112969103e-01
2.2824714139e+00 2.4248309486e-01
2.2988920715e+00 2.4372720592e-01
2.3153127292e+00 2.4486114256e-01
2.3317333868e+00 2.4588409784e-01
2.3481540445e+00 2.4679533917e-01
2.3645747021e+00 2.4759420805e-01
2.3809953598e+00 2.4828011982e-01
2.3974160174e+00 2.4885256340e-01
2.4138366751e+00 2.4931110113e-01
2.4302573327e+00 2.4965536857e-01
2.4466779904e+00 2.4988507433e-01
2.4630986480e+00 2.5000000000e-01


==> header.tex <==
\usepackage{generic}

\usepackage{textcomp}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

% References
\usepackage{csquotes}
\usepackage[english]{babel}

% Algorithms
\RequirePackage{algorithm,algpseudocode}
\algnewcommand\algorithmicinit{\textbf{Init:}}
\algnewcommand\Init{\item[\algorithmicinit]}
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}

% tables
\usepackage{booktabs}
\usepackage{multirow}

% Math packages
\usepackage{dsfont}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{amsfonts}
\usepackage{amsmath}
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}
\usepackage{mathtools}

% Fonts
\let\Bbbk\relax
\usepackage[cmintegrals,cmbraces,varbb]{newtxmath} % Math font
\usepackage[cal=cm,bb=ams]{mathalpha} % Improve calligraphic and bb math
\renewcommand{\ttfamily}{\fontencoding{T1}\fontfamily{lmtt}\selectfont}

% Additional math options
\usepackage{xspace}

% Figures
\usepackage{graphicx}
\usepackage{caption}

% theorems
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{lemma}{Lemma}
\theoremstyle{definition}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}

% Math commands
\DeclareMathOperator*{\argmin}{arg\,min}

% Project-specific definitions
\newcommand{\Rpp}{\R_{>0}}
\newcommand{\Np}{\N_{>0}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rx}{\mathbb{R}^{n_x}}
\newcommand{\Rp}{\mathbb{R}^{n_p}}
\newcommand{\Rn}{\mathbb{R}^{n}}
\newcommand{\Ru}{\mathbb{R}^{n_u}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\PPP}{\mathscr{Y}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\J}{\mathcal{J}}
\renewcommand{\L}{\mathscr{L}}
\newcommand{\p}{\bar{p}}
\newcommand{\PP}{\mathscr{P}}
\newcommand{\mpc}{\mathrm{MPC}}
\newcommand{\tto}{\rightrightarrows}

\renewcommand{\P}{\mathscr{P}}

\usepackage{xcolor}

% Hyperlinks and referencing
\makeatletter
\let\NAT@parse\undefined
\makeatother
\usepackage[hidelinks]{hyperref}
\usepackage[sort]{cleveref}

% Clever ref names
\crefname{appendix}{Appendix}{Appendices}
\AtBeginEnvironment{appendices}{\crefalias{section}{appendix}}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{theorem}{Theorem}{Theorems}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{section}{Section}{Sections}
\crefname{proposition}{Proposition}{Propositions}
\crefname{equation}{}{}
\crefmultiformat{equation}{(#2#1#3}{, #2#1#3)}{, #2#1#3}{, #2#1#3)}
\crefrangeformat{equation}{(#3#1#4-#5#2#6)}
\crefrangeformat{assumption}{Assumptions #3#1#4-#5#2#6}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{subsection}{Subsection}{Subsections}
\crefname{paragraph}{Paragraph}{Paragraph}
\crefname{figure}{Figure}{Figures}
\crefname{table}{Table}{Tables}
\crefname{remark}{Remark}{Remark}
\crefname{example}{Example}{Example}
\crefname{table}{Table}{Table}
\crefname{definition}{Definition}{Definitions}
\crefname{remark}{Remark}{Remarks}

% Add vertical lines in algorithms
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{groupplots}
\usepackage{hf-tikz}
\usetikzlibrary{tikzmark}
\usetikzlibrary{calc}
\usepackage{etoolbox}
\errorcontextlines\maxdimen
% begin vertical rule patch for algorithmicx (http://tex.stackexchange.com/questions/144840/vertical-loop-block-lines-in-algorithmicx-with-noend-option)
% note that some of the packages above are also needed
\newcommand{\ALGtikzmarkcolor}{black}% customise this, if you want
\newcommand{\ALGtikzmarkextraindent}{4pt}% customise this, if you want
\newcommand{\ALGtikzmarkverticaloffsetstart}{-.75ex}% customise this, if you want
\newcommand{\ALGtikzmarkverticaloffsetend}{-.5ex}% customise this, if you want
\makeatletter
\newcounter{ALG@tikzmark@tempcnta}
\newcommand\ALG@tikzmark@start{%
    \global\let\ALG@tikzmark@last\ALG@tikzmark@starttext%
    \expandafter\edef\csname ALG@tikzmark@\theALG@nested\endcsname{\theALG@tikzmark@tempcnta}%
    \tikzmark{ALG@tikzmark@start@\csname ALG@tikzmark@\theALG@nested\endcsname}%
    \addtocounter{ALG@tikzmark@tempcnta}{1}%
}
\def\ALG@tikzmark@starttext{start}
\newcommand\ALG@tikzmark@end{%
    \ifx\ALG@tikzmark@last\ALG@tikzmark@starttext
        % ignore this, the block was opened then closed directly without any other blocks in between (so just a \State basically)
        % don't draw a vertical line here
    \else
        \tikzmark{ALG@tikzmark@end@\csname ALG@tikzmark@\theALG@nested\endcsname}%
        \tikz[overlay,remember picture] \draw[\ALGtikzmarkcolor] let \p{S}=($(pic cs:ALG@tikzmark@start@\csname ALG@tikzmark@\theALG@nested\endcsname)+(\ALGtikzmarkextraindent,\ALGtikzmarkverticaloffsetstart)$), \p{E}=($(pic cs:ALG@tikzmark@end@\csname ALG@tikzmark@\theALG@nested\endcsname)+(\ALGtikzmarkextraindent,\ALGtikzmarkverticaloffsetend)$) in (\x{S},\y{S})--(\x{S},\y{E});%
    \fi
    \gdef\ALG@tikzmark@last{end}%
}
% the following line injects our new tikzmarking code
\apptocmd{\ALG@beginblock}{\ALG@tikzmark@start}{}{\errmessage{failed to patch}}
\pretocmd{\ALG@endblock}{\ALG@tikzmark@end}{}{\errmessage{failed to patch}}
\makeatother
% end vertical rule patch for algorithmicx

\newcommand\xqed[1]{%
  \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
  \quad\hbox{#1}}
\newcommand\demo{\xqed{$\triangle$}}

\usepackage{cite}
\usetikzlibrary{spy}

% custom ref commands for problems
\newcommand{\probone}{\ref{eq:P1}\xspace}
\newcommand{\probtwo}{\ref{eq:P2}\xspace}
\newcommand{\probthree}{\hyperref[eq:P3]{$P_3$}\xspace}
\newcommand{\longprobthree}{\ref{eq:P3}\xspace}

% read data from dubins results
\pgfplotstableread{Figures/Data/dubins_errors.dat}\dubinsErrors
\pgfplotstableread{Figures/Data/dubins_scaling.dat}\dubinsScaling
\pgfplotstableread{Figures/Data/dubins_theta3.dat}\dubinsThetaThree
\pgfplotstableread{Figures/Data/dubins_times.dat}\dubinsTimes
\newcommand{\dubinsval}[4][sci,precision=1]{\pgfplotstablegetelem{#3}{#4}\of{#2}\pgfmathprintnumber[sci zerofill,#1]{\pgfplotsretval}}
\newcommand{\dubinsraw}[3]{\pgfplotstablegetelem{#2}{#3}\of{#1}\pgfplotsretval}

% Data exported by 2_nlp_mpc_overactuated.py (export_dat) -- paths relative to the main .tex file
\pgfplotstableread{Figures/Data/fig3_sensitivity.dat}\figthreetable  % t, dx1_fd, dx2_fd, dx1_proj, dx2_proj, ...
\pgfplotstableread{Figures/Data/mpc_instances.dat}\figthreedegtable  % t, dim_P, dim_U, ...

% linestyles and colors
\definecolor{chocolate2168224}{RGB}{216,82,24}
\definecolor{darkcyan0113188}{RGB}{0,113,188}
\definecolor{purple12546141}{RGB}{125,46,141}

\definecolor{brown1611946}{RGB}{161,19,46}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}

\definecolor{newOrange}{RGB}{255, 127, 14}
\definecolor{newRed}{RGB}{214, 39, 40}
\colorlet{newBlue}{darkcyan0113188}
\definecolor{newlblue}{RGB}{77,190,238}

\pgfplotsset{line4/.style={
    ultra thick,
    newBlue,
    mark=square*, 
    mark size=0.75, 
    mark options={solid}
}}
\pgfplotsset{line5/.style={
    very thick,
    newOrange
}}
\pgfplotsset{line6/.style={
    very thick,
    newRed,
    dash pattern=on 5.25pt off 1.75pt on 1.75pt off 1.75pt,
    mark=*,
    mark size=0.625,
    mark options={solid}
}}

% \newcommand{\rvv}[1]{{\color{newBlue}#1}}
\newcommand{\rvv}[1]{#1}

\usepackage{booktabs}
\usepackage{pgfplotstable}
\newcount\rhoexp

\newif\iffull
\fullfalse

\usepackage{balance}
